Design of Fuzzy Logic Parameter Tuners for Upper-Limb Assistive Robots

Assistive Exoskeleton Robots are helping restore functions to people suffering from underlying medical conditions. These robots require precise tuning of hyper-parameters to feel natural to the user. The device hyper-parameters often need to be re-tuned from task to task, which can be tedious and require expert knowledge. To address this issue, we develop a set of fuzzy logic controllers that can dynamically tune robot gain parameters to adapt its sensitivity to the user's intention determined from muscle activation. The designed fuzzy controllers benefit from a set of expert-defined rules and do not rely on extensive amounts of training data. We evaluate the designed controllers with three different tasks and compare our results against the manually tuned system. Our preliminary results show that our controllers reduce the amount of fighting between the device and the human, measured using a set of pressure sensors.

==> extra.tex <==
%The inputs to the fuzzy controller that tunes the dominant gain consist of the human intention $I_h$ and the dominant gain $E_d$. This controller outputs $\delta E_d$, the amount of change in $E_d$ to be set by the device. The inputs to the fuzzy controller that tunes the opposing gain consist of the human intention $I_h$ and the effort difference $\Delta E$. This controller outputs $\delta E_o$, the amount of change in $E_o$ to be set by the device.





%The rule base consists of six rules and is shown in Table I. It's control surface can be seen in (Fig.~\ref{fig:3})


%Three Gaussian fuzzy sets for each input variable and three
%constant outputs are defined. The constructed rule base of
%the system comprises nine rules. The rule base is complete,
%continuous, and consistent, and is reported in Table I.




%on the device more or less sensitive depending on factors of the users movement by altering the gain parameters. 
%These factors include the human intention, current dominant gain, and the delta effort. 
%The controller was also broken into two parts one controlling the change in dominant gain and the other controlling the opposing gain.

%These factors are the intention of the user, the delta effort, and the current state of the gain parameter on the device. Depending on the intention of the user one of two fuzzy logic rule sets will be chosen. One of the rule sets aims to alter the dominant and opposing gain values based on the current values of the dominant gain and delta effort when the user is moving. These rules will make the dominant effort more sensitive if need be and the opposing effort more resistant if it is too sensitive to make movement smoother. The other rule set shifts the device in a "safe zone" depending on the delta effort. This rule set will make the device more resistant if the device is drifting slightly while the user is trying to hold their joint still. This causes a vibration that the user can feel on their upper arm. The rule set aims to stop this from happening. After that the device will adjust the gain and then repeat this task until the user has completed their use of the device. 


%\begin{figure}
%    \centering
%    \includegraphics[scale=0.5]{flowchart.png}
%    \caption{A flowchart of the algorithm.}
%    \label{fig:4}
%\end{figure}

%\FloatBarrier

%\subsection{Determining Human Intention}

%For the controller what the user is trying to do needs to be determined. The three different actions the user can be preforming are: opening the joint (tricep activation), closing the joint (bicep activation), and not moving at all (no activation). To determine which one of these actions the user is preforming some information from the device can be checked through a serial string that is transferred over Bluetooth. The things that need to be checked are the current position, bicep effort, and tricep effort. Depending on the position compared to the previous position and the current state of the effort values the intention can be determined. The position is checked to know what direction the user is moving in. The efforts are checked to see if the sensors are reflecting the intention. How each intention is determined is shown below:
%\begin{itemize}
%    \item \textit{Opening the Joint / Tricep Activation:} If the position is less then the previous position and the tricep effort is greater then or equal to 25.
%    \item \textit{Closing the Joint / Bicep Activation:} If the position is greater then the previous position and the bicep effort is greater then or equal to 25.
%    \item \textit{No Movement:} If the position is the same as before and if both bicep/tricep efforts are less then 25.
%\end{itemize}

%\subsection{Fuzzy Logic Controller}

%As mentioned the Fuzzy Logic Controller is broken into two. One for altering the dominant gain and the other for the opposing gain. The controllers output a value to change the gain by. Both of the parts are TSK fuzzy systems [2] and used the weighted average of all rule outputs as a defuzzier. 

%The controller that deals with altering the dominant gain takes two inputs the human intention and the current dominant gain. The human intention is either \textit{still} or \textit{movement} which can be either opening or closing the joint. This input is defined by two Gaussian fuzzy sets. The other input is current dominant gain which has a range of [1, 20]. If the gain is \textit{resistant} then it is closer to the lowest value of 1. If it is \textit{normal} then it is closer to the default value of 10. Finally, if it is \textit{sensitive} then it is closer to the max value of 20. This input is defined by having three Gaussian fuzzy sets. The output of this part is five constant values that represents the change to make to the gain value. The output range is between [-3, 3] where -3, -1, 0, 1, 3 correspond to a decrease, small decrease, stay the same, small increase, and increase. The rule base consists of six rules and is shown in Table I. It's control surface can be seen in (Fig.~\ref{fig:3})

%The other part of the controller effects the opposing gain. This part has two inputs which are the following, human intention and delta effort. The human intention is the same as from the other part. The delta effort is defined by the following. It's range is between [-100, 100]. The delta effort is used to determine what sEMG sensor is most effecting the current movement. If it is below 0 then it is consider \textit{opposing}. When it is above 0 it is considered \textit{dominant}. If it is around 0 then it is considered co-contraction. The input is defined by having three Gaussian fuzzy sets. The output is the same as the other one. There are six rules for this and they are shown in Table II. It's control surface can be seen in (Fig.~\ref{fig:3})

%\begin{table}[h]
%\caption{Fuzzy Rule Base for Delta Opposing Gain.}
%\label{Movement Rules}
%\begin{center}
%\hskip-0.5cm\begin{tabular}{|c|c|c|c|}
%\hline
%\vspace{0px} & Dominant & Co-contraction & Opposing\\
%\hline
%Movement & Decr. & Sm. Decr & Same\\
%\hline
%Still & Decr. & Decr. & Same.\\
%\hline
%\end{tabular}
%\end{center}
%\end{table}




%Data would be collected for each state for thirty seconds and once complete and once complete the subject would be given a short rest period to minimize the possibility of fatigue. 





%To confirm that the fuzzy controller was effective at tuning the device during movement we ran some experiments that would encompass doing three tasks while the controller was active and not. To measure if it was effective or not we attached two pressure sensors to the device that would detect if the user was fighting with the device.






%For our research the max EMG was always set to a fixed 100 for both biceps and triceps. 

%Besides choosing a movement type, there are two parameters that users can change to tune the device to their needs. These parameters are the bicep/tricep effort thresholds and the bicep/tricep gain. Whenever the delta effort surpasses the set effort threshold for the muscle of the dominant effort the device will then move in that direction. The effort thresholds can be set to either by between 10 and 100 however, the MyConfig application, a program developed by Myomo that is used to set settings for the device, the effort thresholds can only be set between 10 and 65. Gain is the amplification that the EMG signal receives through the hardware. This parameter can be set between 0.2 and 20. The default value that we also chose for this parameter is 10. A diagram (Fig.~\ref{fig:2}) that the MyConfig shows on the settings screen is shown below to better show these concepts graphically.

%\begin{figure}
%    \centering
%    \includegraphics[scale=0.25]{figures/config.PNG}
%    \caption{The MyConfig dual mode configuration GUI. a) The yellow circle displays the delta effrot. b) The lines labeled bicep and tricep represent the speed once the delta effort passes starts climbing the line the motor will activate in that direction. c) These slides control the effort threshold. d) These sliders control the dual mode parameters. }
%    \label{fig:2}
%\end{figure}
%%% up to here 

%To collect data, the subject wearing the device would preform the task in three different states: when the effort threshold is sensitive which is it being the lowest it can be at 10, normal where the effort thresholds were 20, and finally resistant when the effort thresholds are high being at 40. Without the controller tuning the EMG sensitivity movement should be doable during the sensitive and normal experiments. However, with the effort threshold high sometimes movement can get more difficult. Data would be collected for each state for thirty seconds. Once complete the user would be given a minute to relax. Due to the device being relatively heavy the subject would take off the device after a few tests and take a small break to ensure that fatigue would not effect performance.  


